CommonCanvas: An Open Diffusion Model Trained with Creative-Commons Images

We assemble a dataset of Creative-Commons-licensed (CC) images, which we use to train a set of open diffusion models that are qualitatively competitive with Stable Diffusion 2 (SD2). This task presents two challenges: (1) high-resolution CC images lack the captions necessary to train text-to-image generative models; (2) CC images are relatively scarce. In turn, to address these challenges, we use an intuitive transfer learning technique to produce a set of high-quality synthetic captions paired with curated CC images. We then develop a data- and compute-efficient training recipe that requires as little as 3% of the LAION-2B data needed to train existing SD2 models, but obtains comparable quality. These results indicate that we have a sufficient number of CC images (~70 million) for training high-quality models. Our training recipe also implements a variety of optimizations that achieve ~3X training speed-ups, enabling rapid model iteration. We leverage this recipe to train several high-quality text-to-image models, which we dub the CommonCanvas family. Our largest model achieves comparable performance to SD2 on a human evaluation, despite being trained on our CC dataset that is significantly smaller than LAION and using synthetic captions for training. We release our models, data, and code at https://github.com/mosaicml/diffusion/blob/main/assets/common-canvas.md

==> iclr2023/section/99-scratch.tex <==
\newpage
\input{iclr2023/section/991-outline}
\input{iclr2023/section/992-intro-notes}
\input{iclr2023/section/993-prelim-notes}
\input{iclr2023/section/994-synthetic-notes}
\input{iclr2023/section/995-results-notes}
\input{iclr2023/section/996-rw-notes}
\input{iclr2023/section/997-discussion-notes}
\input{iclr2023/section/998-figures-notes}
\input{iclr2023/section/999-future-notes}

%Even if an image is a worth 1000 words, even if you had a thousand words, you could create a thousand images.

==> iclr2023/section/991-outline.tex <==
\section{Outline}
    
\begin{enumerate}
    \item We train Stable Diffusion 2 on 5\% of the training data as the original and achieving matching FID on MsCoco~\cite{lin2014microsoft}. We also demonstrate that diffusion models can be trained using as little 0.5\% of the training data used in the original model.
    \item We release our dataset of Creative Commons-licensed captioned image as a standard, stable, downloadable, benchmark to evaluate diffusion model consisting over more than 100TB of data and over 70 million captions. %and demonstrate for the first time that synthetic captions can be used to create viable diffusion models without using any copyrighted data, all while matching previously reported metrics.
    % \item We release a higher resolution of YFCC100M that includes images in their original resolution, including images that are more than 4K in resolution.
    \item We reduce the training time of Stable Diffusion 2 by 2.8X through various training pipeline and recipe improvements, allowing practitioners to train the model from scratch for approximately 20,000 A100 hours. This reduction in training time and cost has allowed us to perform rapid experimentation on diffusion models and run the ablation featured in this paper.  %We demonstrate MLSys contributions that can be used to reduce the cost of Stable Diffusion to under \st{\$50,000} \$30,000 dollars.
    % \item We discover evidence absence of scaling laws for the amount of data in a diffusion model and find that while increasing the amount of the data does appear to increase coverage of the model, it does not improve the results on many standard benchmarks. \jc{i find this claim kind of sus. unless we've tried extensive hyperparameter/model parameter scaling experiments, we might just be underfitting the data}
    . % We find that we can outperform a dataset more then 10X larger on FID metrics on Coco.
    %\item We show that uncaptioned data can be integrated into diffusion models through caption models.% and by smartly leveraging caption https://www.overleaf.com/project/64c2d9d675e0f95f732c9628dropout.
    % \item We release our dataset of open captioned data as a standard benchmark to evaluate with diffusion model. Copyrighted image data cannot be redistributed and requires the dataset to be redownloaded. We hope that this dataset becomes the standard large scale captioning datasets like ImageNet and OpenWebText.
    \item We demonstrate how synthetic captions on uncopyrighted data can provide privacy preserving and trademark benefits over web scraped captions. An emergent property of this training scheme is that the proper nouns are replaced by common nouns providing significant privacy benefits, make it significantly more difficult to generate specific people in the training data.

% Dataset - Eval / Dataset - Train
% Model Artifact
% Training Process
    
\end{enumerate}

\begin{enumerate}
    \item Context: 1-2 sentences to set context. Describe the current state of things.
    \begin{enumerate}
        \item Diffusion models work really well and are used a lot.
    \end{enumerate}
    \begin{itemize}
        \item Problem: What is the problem with the current state of things?
    \end{itemize}
    \begin{enumerate}
        \item However, they are trained on large datasets that often contains has copyrighted material, and may infringe on existing laws.
        \item Also, the datasets they are trained on are very large and training models is expensive.
        \item Existing methods: What have people tried to address the problem?
        \begin{enumerate}

        \item \textbf{Exclude copyrighted images manually?}
        \begin{enumerate}
            \item It is impossible to know what is copyrighted unless the author specifies it so this is not possible at the moment. There are web scrape work which tries to only whitelist copyright data, but none of them have been published yet (I am aware of two projects). Openverse originally tried to do this, but realized it wasn't worth there time so instead focused on whitelisting sources.
        \end{enumerate}
        \item \textbf{Delete copyrighted knowledge from the network after training?} 
        \begin{enumerate}
            \item This is actually not viable currently. There are some experimntal results, but they don't match scrutiny
        \end{enumerate}
        \item \textbf{Train on corrupted data?}
        \begin{enumerate}
            \item  There is some work on this. In terms of intent it is the closest thing to what we want to do. Techinically, and in terms of machine learning, it is really cool. In practice, this is not legally defensible at all.
            
        \end{enumerate}
        \end{enumerate}
    \end{enumerate}

    \item Limitations: Why do the existing methods fail?
    \begin{enumerate}
        \item It’s impossible to comb through large datasets by hand
        \item It’s not possible to prune all the copyrighted information from the network for some reason (see above)
        \item Training on corrupted data is not legally defensible. It's not transformative in the slightest.
    \end{enumerate}
    \item Proposed approach - Structured Label Distillation
    \begin{enumerate}
        \item We propose [label distillation / label transfer / model transfer / …], a technique for transferring knowledge from a small high-quality dataset to another large, unlabeled dataset.
    \end{enumerate}
    
\item We produce a new and high quality synthetically labeled dataset by instantiating this technique in the context of diffusion models we train on this dataset using efficiency techniques. This is legally better than any paper trained before that does not use Wikimedia or compensated AMT folks. It's as good as it's going to be.


    \item Comparison to existing work: How does it solve the problem differently from existing work and why is it better?
    \begin{enumerate}
        \item 
We don’t need to manually delete data points or facts from inside the model: we start with a copyright-free dataset to begin with.
\item We don’t need to corrupt data, hence our data is better quality. Also corrupted data is still liekly to be copyrighted.
    \end{enumerate}

    \item We take the angle of distillation/transfer, but our technique is different
    \begin{enumerate}
        \item Model distillation: distills big model into smaller model, not the same
        \item Dataset distillation: distills large number of x’s into smaller x’s; we distill y’s
        \item Domain Transfer: I know there is some work on transfer too… (here, a lit review is really important)
    \end{enumerate}

    \item Technical innovation: Why is this approach non-trivial? What were the key technical insights that were need to make the approach work. Write key insights as bullet points.
    \item Non trivial because it’s not clear if synthetic labels will be good enough. Also not clear if this will be computationally feasible.
    \item Key innovations are:
    \begin{enumerate}
        \item Use of a transfer model: We use a high-quality model to transfer labels.
        \item Scaling innovations. We use less date and make the model more efficient to train
        \item (We don't want LLM regularization to be part of the method.)
        \item We use synthetic captions for the first time and show them to be effective
    \end{enumerate}
    
    \item What experiments do we have / Could we have. Clean up and explaine?
    \begin{enumerate}
    \item MSCoco FID
    \item Scaling behavior on MSCoco FID
    \item Local Narrative (Open Images) dataset - CLIP/FID
    \item Celebrity Identification (MS-CELEB-1M) - classifier based
    \item Metrics on Google WIT dataset?
    \item N-GRAM Diversity vs CLIP SCore of captions
    \item Zero Shot - Eval on ImageNet % N-FOLD FID calculation <=> metric / Try on ImageNet? MS-Celeb
    \item CLIP Score + FID + KID + CLIP-FID on COCO2014
    \item Human evaluation on parti prompts
    \item CLIP/FID eval on conceptual captions subsests?
    \item Find a mascot dataset?
    \item FineTune (Likely Post Rebuttal)
    \begin{enumerate}
        \item Finetune on Anime? Met Art Dataset
        \item MetFaces dataset -> Sg2
        \item INaturalist
        \item Danbooru 
    \end{enumerate}
    \end{enumerate}
\end{enumerate}

LLM regularization…?
@Aaron Gokaslan
 this is like how in the LeND paper we have: (1) vector-valued noise, (2) instance-conditioned noise; (3) aux var conditioning
Evidence: what results (experiments on theoretical analysis) do we have that the proposed approach solves the method better than existing work?
Name key metrics: how do you evaluate that you do not infringe on copyright
Name baselines
Name datasets and summarize results
Other advantages: add lesser benefits of the method that important to highlight
We use less data, we establish scaling laws, etc.
We release datasets and models

==> iclr2023/section/992-intro-notes.tex <==
\section{Introduction}
\begin{itemize}[topsep=0pt, leftmargin=.5cm]
    %\item I think the main story that should be emphasized is the MLSys one, and perhaps we should go all-in on datasets as the main focus. %This paper takes a data-centric ML approach to evaluating possibilities and trade-offs for training diffusion models, under a whole host of settings/ considerations that modern large-scale datasets raise. To list a few: 
    \item \textbf{Motivation}: Lawsuits, ethical rational. There are good reasons to try to train on public-domain images (legal rationale, ethical rationale).; could make the point that this key to opening up access to models responsibly. 
    \item \textbf{This is a great motivation, but has two huge unsolved technical problems.} But, this comes with its own challenges that are data-centric ML and MLSys-flavored. 
    \begin{itemize}
        \item For one, public-domain images are a scarcer resource than web-scraped stuff we're hoping to compete with. This means an inherently smaller training dataset, in a setting where folk wisdom says that more data is better.
        \item And, there are no captions. So there is a data completeness/ quality problem.
    \end{itemize} 
    \item We study and address both of those problems. 
    \begin{itemize}
        \item 1) We actually don't have to train with a lot of data; and we can also get additional speed-ups, and make things even more efficient, more-widely accessible. The efficiency stuff beyond the data thing isn't that novel from a research perspective, so I think we shouldn't focus too hard on it here. We should focus mostly on the parameter saturation argument.
        \item This means that, at least in theory, we should be able to train a decent CC model on the number of images we have. But..what do we do about the captions.
        \item 2) Why derive a novel technique (concurrent with other work, but slightly different), which we call \textbf{blah; create macro}.
    \end{itemize}
    %\item On the flip side, if we can solve the above to problems, there's a kind of have-your-cake-and-eat-it-too story. If we can get this to work well, we simultaneously decouple from datasets (at least directly) that have currently come under a lot of heat with respect to IP, and, we'd be making training more efficient (and thus opening up new research possibilities for those who are more resource-constrained than the largest companies). 
    %\item This is what we explore in this paper. We ask, is it possible to train a competitive stable diffusion model on a corpus of un-captioned public-domain images that is 10\% the size of LAION? (or something like that as the main question) 
    % \begin{itemize}
    %     \item Models are getting bigger and bigger, as a function of larger and larger datasets. And as a result, they're getting more expensive to train. (and, in fact, this is intractable for a lot of potential model trainers, who aren't at a handful of companies) 
    %     \item The large datasets that these models are trained on have a lot of problems associated with them. We'll highlight two. In the text-to-image modality, captions are really crap (e.g., LAION captions. There are data quality issues. Second, even if we can get decent performance in spite of such data quality issues, it's increasingly under scrutiny whether it is legal or ethical to scrape and train. Tons of lawsuits, lots of open questions about copyright and IP. Even if we can / it ends up being legal, should we be doing this? (There's a lot of debate in the community on this). An alternative is licensing datasets. Again, there are issues of cost there (per-image licenses?) 
    % \end{itemize}
    % \item In short, generative-AI research has a data problem. For one, it is really hard to do research that involves pre-training on state-of-the-art models, without massive infrastructure investment, etc. On the other, even if we do have that infrastructure, there are other issues with the data that we increasingly care about.
    \item The answer to this question is nuanced, but the short answer is that we can train a really effective(?) diffusion model on public domain image corpus with 80M examples, synthetic captions that we generate for them. 
    \item The longer answer is we learned a lot of things by trying to do this, expose interesting trade-offs, clear questions for future research in multiple directions. For example, we are able to train a surprisingly good model; in some cases, out-performs; in others, does not do as well; but, this can also be a good thing, has the affordance of being better wrt PII. 
    \item In summary, we do three things:
    \begin{itemize} 
        \item Explore data efficiency stuff wrt LAION; try to get a sense of trade-off space / MLSys story of training on less data. And we have some surprising findings here: No difference in performance compared to training on the whole dataset (Section 3)
        \item This suggests that indeed worth attempting our initial goal, of training on a public-domain dataset of same size. To do this, generate synthetic captions (Section 4) 
        %\item Training data size reduction story re: LAION. (This is useful in itself, and warrants additional research for those that can afford to do ablation studies on what's going on here with stable diffusion.)
        %\item And, since this is possible, can we instead swap out LAION for a dataset of similar size that is instead made up of public-domain images? And the answer is we can, and we can get suprisingly good performance (with some nuance). But of course, images are only half the story for text-to-image models. We also need captions. For this, we create synthetic captions for the public-domain images. (And then this story is a bit more complicated / needs more nuance because we generate the captions using a model that was trained on data we're calling a problem; but, we can make the case that this is still better / less of a problem and a good starting point, because we're making data (captions) that have a higher threshold for being copyrightable (tons of lit on this; defer to experts) as a function of their size; still potentially copyrightable expression in captions, but not of the same kind as artistic images, full-length text, etc. This is mostly Appendix material, with a short summary in the related work or later). A side-effect / benefit of this is we do better with respect to PII, other problems that people are concerned about with respect to deepfakes that involve real people (pull up Levendowski, etc. on this); other problems that aren't just copyright from using pictures of real people, and this in part solves that. 
        \item Run series of experiments to evaluate performance. Release all the artifacts (model, dataset, benchmark) for others to use. Expose the trade-off space (as described above) with respect to less data, not using copyright images to train. This should be one of the benchmarks people use when they test their models, do research on diffusion models, etc (Section 5).
    \end{itemize}
\end{itemize}

%\begin{enumerate}
%     \item No Copyrighted Data in -> No Copryighted Data Out.
% Copyright violation requires copying.
% If the model can recreate it, without having seen it, then it's probably not copyrightable in the first place

% Caption -> Generator.
% Captions are not copyrighted

% Transformative Use

% Make the argument Fixation

% Add human analogy.

% CAPTIONs are NOT COPYIRGHTABLE
\cooper{Human-authored captions are copyrightable. Computer-generated ones, however, are not.}

The image from which the caption copyrighted
%\end{enumerate}

==> iclr2023/section/993-prelim-notes.tex <==
\section{Background + Motivation}

% \begin{enumerate}
%     \item TODO: Add background about Stable Diffusion
%     \item TODO: Add background about why LAION is bad
% \end{enumerate}
Recently, large caption datasets such as LAION has enabled impressively large and expressive diffusion models such as Stable Diffusion to be produced~\cite{rombach2022diffusion}. However, only a few models have been trained on this scale of data due to the massive cost of training the models. Furthermore, even fewer of these models have been released due to the uncertain legal nature of these models.

%In this paper, we strive to minimize the legal risk of these models, and by doing so propose caption grafting to transfer label knwo

%Few large scale diffusion models have been open-sourced due to the legal risks of a large caption datasets such as LAION-5B. Reproducing data from training data in this domain represents significant legal risk. \aaron{COoper Please cite more here.}

\begin{figure}
\includegraphics[width=\textwidth]{iclr2023/figs/charts/diffusion-cat-compare.png}
\label{fig:conceptual-captions-benchmark}
\caption{Ablation plot where we go from LAION+LAION captions -> LAION+BLIP2 captions -> YFCC+BLIP2 captions at equivalent number of samples (pin to size of YFCC?) at 256x256}
\end{figure}

\cooper{This feels like method/ related work material}
Captions are an extremely expensive and difficult type of annotation to collect. Prior work has focused on trying to extract them automatically from webpages and assistive text. However, these captions are often low quality, machine-generated, or correspond to product descriptions more often than they do to hand written text. Furthermore, prior work on diffusion model have used billion of image caption pairs to train these models. Do we actually need these many images to train these models? Furthermore, how does the number of images influence the performance of the models? 

%\textbf{Creative Common Images are Rare}

%Something that is even more rare than image captions are images that are known to be in the public domain. Openverse~\cite{}, a creative commons search engine, only lists approximately 700 million such images known to exist. Of those, very few of them have captions. When OpenAI trained the CLIP~\cite{} model, they were only able to source 14,829,396 images that had either used provided captions, or the titles were deemed descriptive enough to likely be captions. However, compared to caption datasets like DataComp~\cite{gadre2023datacomp} that the available amount of Creative Common images is between 1 and 10\% of the captioned data. Well captioned data is even more rare, and data that are safely commerically usable are even more rare. Furthermore, even if all the URLs and captions are easily distributed, link rot ensures that it is impossible to compare results between different models even if they are trained on the same dataset. 

%\textbf{LinkRot is a huge problem}

%When downloading LAION-2B for the our paper, we were unable to download nearly half of the images less than 1 year after release! This observation suggests that large scale caption datasets often have fairly short half-lives. 

%\textbf{Commerically usable creative common images are also rare}

%This motivates our first contribution, the creation of a dataset of creative common images AND captions that can be used to train a public domain diffusion model.


%There are two problems with this approach though, firstly, the number of public domain images 

%Therefore, the problem setup is as follows. We have 1 domain that we cannot use directly for training, however, that data 



\


\subsection{Are Diffusion Models over trained? Can we get the same performance with less data?}

Due to the cost of training diffusion models, little exploration has been done in how these models scale with new data amounts of data. The more unique data that is added into a model, the more rare concepts it can represent. However, the question remains: Does the distribution of training data actually match human-generated captions? MSCoco is one of the most studied datasets consisting of user-generated captions, and diffusion models are often compared to it. \cooper{This seems like something that should go in results? That way we can talk about other splits as something cool you all did?}

\textbf{Model Capacity Problem}
. 
\begin{enumerate}
    \item If you calculate the compression ratio of the model, a reasonable model would store something like 256k images, but this is attempting to store 1 billion which which 4-5 magnitudes off! This suggests that the model needs to be much larger, which other work such as SDXL~\cite{podell2023sdxl} has shown helps, but 
    \item Flush out with some math \aaron{Please fill out the math Cory}
    \item 
\end{enumerate}


\begin{enumerate}
    \item SD2 cannot use all the data effectively
    \item We can improve performance by increasing both the width / depth of the model
    \item SDXL's architecture is a bit better.
\end{enumerate}

\begin{enumerate}
    \item LAION has low quality images
    \item LAION has low quality captions
    \item LAION has very few high resolution images
\end{enumerate}

==> iclr2023/section/994-synthetic-notes.tex <==


Synthetic data creation is a well studied problem; however, no works have explored training a large-scale diffusion model with synthetic captions. Prior work has established that training with captions or class labels as a auxiliary training data helps improve the training of other generative models~\cite{}. Furthermore, captions are an important ingredient in being able to control these models efficiently using classifier-free guidance. This poses the question, can we transfer the caption knowledge from a previous protected dataset, LAION to our dataset new public domain dataset. In other words, can we distill the knowledge from this large caption dataset, and then transfer that knowledge to an uncopyrighted data. Our results show, surprisingly, that simply taking a caption model trained on the protected dataset and applying that to our public domain datasets works surprisingly well and yields additional benefits which we explore later in the paper.


% To explicitly separate the two domains—the protected domain and the synthetic domain—let's redefine some general terms: 

% \begin{itemize}
%     \item \( D_{\text{prot}} \) : Protected dataset with original images and captions
%     \item \( D_{\text{unseen}} \) : Dataset of unseen images
%     \item \( D_{\text{syn}} \) : Dataset of synthetic captions corresponding to the unseen images
%     \item \( F_{\text{gen}} \) : Data generation model (trained on \( D_{\text{prot}} \))
%     \item \( F_{\text{main}} \) : Main model (trained on \( D_{\text{unseen}} \) and \( D_{\text{syn}} \))
%     \item \( x_{\text{prot}}, y_{\text{prot}} \) : Data points (image-caption pairs) in the protected domain
%     \item \( x_{\text{unseen}}, y_{\text{syn}} \) : Data points (image-caption pairs) in the synthetic domain
% \end{itemize}

% The generalized process could be described by the following steps:

% \begin{enumerate}
%     \item \textbf{Train the Data Generation Model on \( D_{\text{prot}} \)}
%     \begin{equation}
%     F_{\text{gen}} = \arg \min_{F_{\text{gen}}} L_{\text{gen}}(D_{\text{prot}}; F_{\text{gen}})
%     \end{equation}
%     where \( L_{\text{gen}} \) is the loss function for the data generation task.

%     \item \textbf{Generate Synthetic Captions \( D_{\text{syn}} \) for \( D_{\text{unseen}} \) using \( F_{\text{gen}} \)}
%     \begin{equation}
%     D_{\text{syn}} = F_{\text{gen}}(D_{\text{unseen}})
%     \end{equation}

%     \item \textbf{Train \( F_{\text{main}} \) on \( D_{\text{unseen}} \) and \( D_{\text{syn}} \)}
%     \begin{equation}
%     F_{\text{main}} = \arg \min_{F_{\text{main}}} L_{\text{main}}(D_{\text{unseen}}, D_{\text{syn}}; F_{\text{main}})
%     \end{equation}
%     where \( L_{\text{main}} \) is the loss function for the main model.
% \end{enumerate}


% \begin{itemize}
%     \item \( D_s \) : Source dataset for training the data generation model
%     \item \( D_t \) : Target dataset for the main model
%     \item \( F_{\text{gen}} \) : Data generation model
%     \item \( F_{\text{main}} \) : Main model
% \end{itemize}

% The generalized process could be described by the following steps:

% \begin{enumerate}
%     \item \textbf{Train the Data Generation Model on \( D_s \)}
%     \begin{equation}
%     F_{\text{gen}} = \arg \min_{F_{\text{gen}}} L_{\text{gen}}(D_s; F_{\text{gen}})
%     \end{equation}
%     where \( L_{\text{gen}} \) is the loss function for the data generation task.

%     \item \textbf{Generate Synthetic Data \( D_{\text{syn}} \) for \( D_t \) using \( F_{\text{gen}} \)}
%     \begin{equation}
%     D_{\text{syn}} = F_{\text{gen}}(D_t)
%     \end{equation}

%     \item \textbf{Train \( F_{\text{main}} \) on \( D_t \) and \( D_{\text{syn}} \)}
%     \begin{equation}
%     F_{\text{main}} = \arg \min_{F_{\text{main}}} L_{\text{main}}(D_t, D_{\text{syn}}; F_{\text{main}})
%     \end{equation}
%     where \( L_{\text{main}} \) is the loss function for the main model.
% \end{enumerate}
\begin{enumerate}
    \item 
    Take a captioning model trained on a large copyrighted dataset BLIP2. BLIP2 is a model which uses a frozen image embedding model as well as a frozen large language model and trains a qformer network to link them together. This allows the model to achieve SOTA results on zero-shot captioning.
    \begin{enumerate}
        \item Why BLIP2? SOTA Zero Shot Caption performance on a variety of benchmarks
        \item Add language prior thanks to it's frozen LLM
        \item Can use language model to enhance model to more than original data 
    \end{enumerate}
\end{enumerate}





Creating uncopyrighted captions:
\begin{enumerate}
    \item We use that to caption a large uncopyrighted dataset (YFCC100M, Openverse). None of the inputs to the model at this point are copyrighted; the output is sent through a network trained on copyrighted data, but the output of the model is itself non-copyrighted.
    \begin{enumerate}
        \item YFCC100M is very influential dataset (add citations)
        \item It lacks captions although large parts of it has been captioned. OpenAI even used a 14 million subset and image titles as pseudo captions for CLIP2 experiments
        \item Only a small portition of licensed properly to use in commerical applications, however 400 million images exist in Openverse
    \end{enumerate}
    \item We then train an SD2 architecture using a variety of speedups. First, we pre-compute all the latents from the VQ-VAE used in latent diffusion.
    \item Show that results are comparable. Where do they differ? Why can we not use them?
    \item Describe the Architecture + Method of Training Diffusion Model
\end{enumerate}



%\textbf{}

%The release of Llama by Meta~\cite{} has demonstrated the value of having a large, legally unambiguous, high quality generative model for users to finetune. Within a few weeks, LLAMA2 finetuned models began to dominate various benchmarks. 



Concurrent work by \cite{nguyen2023improving} on creating caption datasets have focused on using synthetic captioning model such as BLIP2 to replace low quality caption data in existing datasets, we take this a step further and see the viability of constructing a dataset consisting solely of synthetically generated captions.

\begin{figure}
    \centering
    \includegraphics{example-image-c}
    \caption{Qualitative Caption Examples? Show the one Landan found?}
    \label{fig:enter-label}
\end{figure}

==> iclr2023/section/995-results-notes.tex <==
\section{Results}

\subsection{What is the performance of Synthetic captions?}

We do reasonably well without training on any copyrighted data. We also show that architectural improvements can compensate for fewer data samples. Furthermore, we observer that as we reduce the number of samples as observed in figure 1, our FID does not increase, in fact, we observe a slight decrease in FID. We replace the LAION captions with synthetic BLIP2 created and observe an average increase of 2.5-5 CLIP-FID. In certain categories such as COCO captions, we actually observe a drop in CLIP-FID.

    % \item Scaling behavior on MSCoco FID (see descaling section)
    % \begin{enumerate}
    %     \item 
    % \end{enumerate}
    \begin{enumerate}
        \item Show that 
    \item Local Narrative (Open Images) dataset - CLIP/FID
        \item Still need to run this experiment. results TBD
        \item Qualitatively, it's really obvious that is't not the same people
        \item Let's include some quantitative experimetns for the rebuttal.
    \item Celebrity Identification (MS-CELEB-1M) - classifier based
    % \item Metrics on Google WIT dataset?
    % \item Zero Shot - Eval on ImageNet % N-FOLD FID calculation <=> metric / Try on ImageNet? MS-Celeb
    \item CLIP Score + FID + KID + CLIP-FID on COCO2014
    \item Human evaluation on parti prompts
    \item CLIP/FID eval on conceptual captions subsests (computed)
    \item Show qualitative examples of trying to generate copyright bait \aaron{Please take care of Cooper}
    \item FineTune (Likely Post Rebuttal)

        \item Finetune on Anime? Met Art Dataset
        \item MetFaces dataset -> Sg2
        \item INaturalist 
        \item Wikimedia - only one with actual captions. WIT
        \item Danbooru 

\end{enumerate}


==> iclr2023/section/996-rw-notes.tex <==
\section{Related Work}

\textbf{The Most Related }

\textbf{Caption Datasets from Social Media}
RedCaps~\cite{desai2021redcaps}

\textbf{Creation Caption Datasets from Unpaired Images and Captions}

The most significant work related to our study is found at \href{https://arxiv.org/pdf/2307.10350.pdf}{here}. The researchers noted that some captions in the datasets are inadequate, yet still useful. They propose a replacement solution with BLIP2, which offers a diversity/quality trade-off.

\textbf{DIME-FM: DIstilling Multimodal and Efficient Foundation Models}

In cases where there are many unpaired sentences that could potentially serve as captions and numerous images that could have captions, linking them becomes a challenging task. The researchers address this issue in their work \href{https://arxiv.org/abs/2303.18232}{here}.

\textbf{Cooperative Distillation}

Another significant work includes a proposal for a new technique, cooperative distillation, which uses both clean curated datasets and web-scale automatically extracted captions, like the Google Conceptual Captions dataset (GCC)~\cite{sharma2018conceptual}. This technique improves the expressiveness of the captions due to the rich vocabulary of the GCC dataset. Details can be found \href{https://arxiv.org/abs/2012.11691}{here}.

\textbf{Ambient Diffusion}

Ambient Diffusion, presented \href{https://arxiv.org/abs/2305.19256}{here}, is a technique that allows learning clean distributions from corrupted data. It ensures that the model never sees the copyrighted data, thus, it cannot copy it.

\textbf{Image Copyright Protection}

The related work on image copyright protection can be found \href{https://www.sciencedirect.com/science/article/abs/pii/S0031320321004659}{here}.

\textbf{Synthetic Images for Caption Data Augmentation}
In \cite{caffagni2023synthcap}, they propose a method to use synthetically generated images to improve the training of a captioning model.

\textbf{Humpback}
One of the most similar work to us is called Humpback~\cite{li2023self} which generates a natural language instruction-tuning dataset by training a model which creates instructions from text. In this case, raw text is extremely cheap, but instructions are not. Likewise, captions are extremely expensive



\textbf{Generalization}
The paper says that diffusion models cannot generate data outside of their training data well, we show this be the case as it does not generate copyrighted concepts nearly as well.\url{https://arxiv.org/pdf/2305.14712.pdf} 


% \textbf{Do Diffusion Models Actually Steal Data?}
% Do diffusion models actually steal from the training distribution? Usually, the training distribution of the model is unknown (even for LatentDiffusion). Here we release the training distribution along with the model, enabling scientists to for the first time confirm whether or not something is in the training set.
% \url{https://arxiv.org/abs/2305.20086}. Just because a prompt can be engineered to reproduce a training image does not mean it was in the training dataset. A.F. Cooper is going to take care of it.
% \begin{enumerate}
%     \item Diffusion models can be thought of denoising autoencoders
%     \item If I autoencoded a copyrighted image, would that count as stealing? No.
% \end{enumerate}


% \section{Problem Setup}
% We are transferring a relationship from two domains in a protected dataset, to an unprotected dataset that we can use during train time.

% \section{Machine Learning Experiment?}

% The question of whether captions outputted by a captioning model are subject to the copyright of the training data used to train the model is a topic of ongoing discussion and research. A number of significant questions remain, such as: Can a formulation for diffusion be established that does not need to condition on time (at least in the v-prediction framework)? Is it possible to encode the raw logits into the model instead of just the captions? How can we guarantee that no visual features are leaking through?

% \section{The Importance of Creative Common Datasets YFCC100M - Major Limitation}

% Finally, an insightful graphic on the importance of Creative Commons datasets can be found \href{https://adam.harvey.studio/creative-commons/}{here}.

% \section{The Importance of a Stable Benchmark}
% Very few large-scale caption datasets are reproducible, and virtually none of the largest ones have static listings of images that can be easily reproduced. Even the LAION dataset have a linkrot of nearly 50\% just a year after it's release.

% \section{Multimodal Distillation}

% We frame this problem as follows: 

% We have a relationship / mapping that we want to learn on a tainted copyrighted dataset, such as an image-to-text mapping, and we want to transfer the knowledge in that model to a new dataset. Recent work has attempted to learn various multimodal embeddings across datasets such as ImageBind by Meta.


==> iclr2023/section/997-discussion-notes.tex <==




Things that would be nice to have:

\begin{enumerate}
    \item fine tuning results (Push to the supplement)
    \item SD2++ + SDXL (SD+2 we will hopefully barely have in time)
\end{enumerate}

\textbf{Performance is significantly better than expected given the limited training data and synthetically generated captions}
\begin{enumerate}
    \item Show that CLIP Score aligns better
\end{enumerate}


\subsection{Practical Cost of Training Models}

Throughout this paper, we have trained these diffusion models from beginning to end multiple times. Stablility AI claimed that training their initial Stable Diffusion-v1 model cost more than \$500,000 in compute costs. We apply several optimizations here to substantially lower our experiment cost and enable efficient fine-tuning\aaron{TODO Cory}:

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{iclr2023/figs/charts/perf-scaling.pdf} 
    \caption{Put speed up bar chart here with the MosaicML Logo removede}
    \label{fig:enter-label}
\end{figure}



==> iclr2023/section/998-figures-notes.tex <==
\begin{figure}

\includegraphics[width=\textwidth]{iclr2023/figs/charts/laion-100m-vs-clip-30m-metrics.png}
\caption{ Training on CC data (YFCC) at large scale with autogenerated captions matches SD performance. \todo{update} }
\label{fig:SD2Compare}
\end{figure}

\begin{figure}
    \centering
    \includegraphics{example-image-a}
    \caption{BLIP2 captions vs original captions cosine similarity (CLIP SCORE) vs diagrams}
    \label{fig:cap-cosine-similarity}
\end{figure}

\begin{figure}
    \includegraphics{example-image-b}
    \caption{Architecture Diagram.}
\end{figure}

% \begin{figure}
%     \centering
%     \includegraphics{example-image-a}
%     \caption{Stable Diffusion into the Blogpost MLSys}
%     \label{fig:enter-label}
% \end{figure}

\begin{figure}
    \centering
    % \includegraphics[width=\textwidth]{iclr2023/figs/mickey-mouse.png}
    % \includegraphics[width=\textwidth]{iclr2023/figs/charts/yfcc-pkm.png}
    \caption{Can you make mickey mouse? Pokemon Gen-1 plot. Redo so its a bit cleaner.}
    \label{fig:mmouse}
\end{figure}


% \begin{figure}
%     \centering
%     \includegraphics{example-image-c}
%     \caption{Use v-prediction, better at night (don't need offset noise?)}
%     \label{fig:night-time}
% \end{figure}


\begin{figure}
    \centering
    %\includegraphics[width=0.45\linewidth]{iclr2023/figs/charts/pie-charts/yfcc100m-license-img.png}
    \includegraphics[width=0.45\linewidth]{iclr2023/figs/charts/pie-charts/flickr-total-licenses-cc.png}
    \caption{Proportion of usable images}
    \label{fig:enter-label}
\end{figure}

==> iclr2023/section/999-future-notes.tex <==
\section{Future Work}
\begin{enumerate}
    \item Work on releasing the rest of Openverse.
    \item Release more open domain images
    \item Can we provide a way to crowdsource captions
    \item Replicate and open source other leading models such as Imagen / SDXL.
    \item Further reduce training cost through architectural improvements like DiT~\cite{peebles2022scalable}.
    \item Scaling up the model (SDXL++)
\end{enumerate}

==> iclr2023/section/outline.tex <==
\textbf{1. Introduction}:
\begin{itemize}[topsep=0pt, leftmargin=.5cm]
    %\item I think the main story that should be emphasized is the MLSys one, and perhaps we should go all-in on datasets as the main focus. %This paper takes a data-centric ML approach to evaluating possibilities and trade-offs for training diffusion models, under a whole host of settings/ considerations that modern large-scale datasets raise. To list a few: 
    \item \textbf{Motivation}: Lawsuits, ethical rational. There are good reasons to try to train on public-domain images (legal rationale, ethical rationale).; could make the point that this key to opening up access to models responsibly. 
    \item \textbf{This is a great motivation, but has two huge unsolved technical problems.} But, this comes with its own challenges that are data-centric ML and MLSys-flavored. 
    \begin{itemize}
        \item For one, public-domain images are a scarcer resource than web-scraped stuff we're hoping to compete with. This means an inherently smaller training dataset, in a setting where folk wisdom says that more data is better.
        \item And, there are no captions. So there is a data completeness/ quality problem.
    \end{itemize} 
    \item We study and address both of those problems. 
    \begin{itemize}
        \item 1) We actually don't have to train with a lot of data; and we can also get additional speed-ups, and make things even more efficient, more-widely accessible. The efficiency stuff beyond the data thing is not that novel from a research perspective, so I think we shouldn't focus too hard on it here. We should focus mostly on the parameter saturation argument.
        \item This means that, at least in theory, we should be able to train a decent CC model on the number of images we have. But..what do we do about the captions.
        \item 2) Why derive a novel technique (concurrent with other work, but slightly different), which we call \textbf{blah; create macro}.
    \end{itemize}
    %\item On the flip side, if we can solve the above to problems, there's a kind of have-your-cake-and-eat-it-too story. If we can get this to work well, we simultaneously decouple from datasets (at least directly) that have currently come under a lot of heat with respect to IP, and, we'd be making training more efficient (and thus opening up new research possibilities for those who are more resource-constrained than the largest companies). 
    %\item This is what we explore in this paper. We ask, is it possible to train a competitive stable diffusion model on a corpus of un-captioned public-domain images that is 10\% the size of LAION? (or something like that as the main question) 
    % \begin{itemize}
    %     \item Models are getting bigger and bigger, as a function of larger and larger datasets. And as a result, they're getting more expensive to train. (and, in fact, this is intractable for a lot of potential model trainers, who aren't at a handful of companies) 
    %     \item The large datasets that these models are trained on have a lot of problems associated with them. We'll highlight two. In the text-to-image modality, captions are really crap (e.g., LAION captions. There are data quality issues. Second, even if we can get decent performance in spite of such data quality issues, it's increasingly under scrutiny whether it is legal or ethical to scrape and train. Tons of lawsuits, lots of open questions about copyright and IP. Even if we can / it ends up being legal, should we be doing this? (There's a lot of debate in the community on this). An alternative is licensing datasets. Again, there are issues of cost there (per-image licenses?) 
    % \end{itemize}
    % \item In short, generative-AI research has a data problem. For one, it is really hard to do research that involves pre-training on state-of-the-art models, without massive infrastructure investment, etc. On the other, even if we do have that infrastructure, there are other issues with the data that we increasingly care about.
    \item The answer to this question is nuanced, but the short answer is that we can train a really effective(?) diffusion model on public domain image corpus with 80M examples, synthetic captions that we generate for them. 
    \item The longer answer is we learned a lot of things by trying to do this, expose interesting trade-offs, clear questions for future research in multiple directions. For example, we are able to train a surprisingly good model; in some cases, out-performs; in others, does not do as well; but, this can also be a good thing, has the affordance of being better wrt PII. 
    \item In summary, we do three things:
    \begin{itemize} 
        \item Explore data efficiency stuff wrt LAION; try to get a sense of trade-off space / MLSys story of training on less data. And we have some surprising findings here: No difference in performance compared to training on the whole dataset (Section 3)
        \item This suggests that indeed worth attempting our initial goal, of training on a public-domain dataset of same size. To do this, generate synthetic captions (Section 4) 
        %\item Training data size reduction story re: LAION. (This is useful in itself, and warrants additional research for those that can afford to do ablation studies on what's going on here with stable diffusion.)
        %\item And, since this is possible, can we instead swap out LAION for a dataset of similar size that is instead made up of public-domain images? And the answer is we can, and we can get suprisingly good performance (with some nuance). But of course, images are only half the story for text-to-image models. We also need captions. For this, we create synthetic captions for the public-domain images. (And then this story is a bit more complicated / needs more nuance because we generate the captions using a model that was trained on data we're calling a problem; but, we can make the case that this is still better / less of a problem and a good starting point, because we're making data (captions) that have a higher threshold for being copyrightable (tons of lit on this; defer to experts) as a function of their size; still potentially copyrightable expression in captions, but not of the same kind as artistic images, full-length text, etc. This is mostly Appendix material, with a short summary in the related work or later). A side-effect / benefit of this is we do better with respect to PII, other problems that people are concerned about with respect to deepfakes that involve real people (pull up Levendowski, etc. on this); other problems that aren't just copyright from using pictures of real people, and this in part solves that. 
        \item Run series of experiments to evaluate performance. Release all the artifacts (model, dataset, benchmark) for others to use. Expose the trade-off space (as described above) with respect to less data, not using copyright images to train. This should be one of the benchmarks people use when they test their models, do research on diffusion models, etc (Section 5).
    \end{itemize}
\end{itemize}
\textbf{2. Background and Motivation}: 
\begin{itemize}[topsep=0pt, leftmargin=.5cm]
    \item Stable Diffusion and LAION background. Include info about model and dataset size, training time (as best as we can find). Issues with captions in the dataset, but at least we have them. 
    \item Scrutiny around LAION, Stable Diffusion (lawsuits); motivation for public domain (why this is something to target) 
    \item Sign post: 2 problems: scarce images, no captions, which we address in turn.
\end{itemize}
\textbf{3. De-Scale Section}: 
\begin{itemize}[topsep=0pt, leftmargin=.5cm]
    \item First thing to do, see if it's viable to even try to train Stable Diffusion with much less data.
    \item Summarize experiments and findings, which are themselves really surprising. Validates that worth trying public-domain-sized training dataset, but also warrants (perhaps) additional exploration on its own. Defer to future work. 
\end{itemize}

\textbf{4. Synthetic Caption Generation Section}: 
\begin{itemize}[topsep=0pt, leftmargin=.5cm]
    \item Signal back to prior section -- there's good reason to try to do this, from an images perspective. What are we going to do about captions?
    \item This is where a formalization would go, if we want one. Also not convinced we need that exactly. We're applying a model to some images; transferring the knowledge from that domain to see if it generalizes well to another (the public-domain images). I'm not sure what math would do to help tell that story. \aaron{I think just having some math that describes what we are doing is fine. We are generally transfering a projection between one domain onto another onto unknown / protected samples of taht domain } How do we evaluate caption quality, other than manually? \aaron{CLIP score is a flawed metric, but it's what people do.} If the answer is manually, then I think we leave it at that and don't try to say anything in a more formal way. \aaron{Provide qualitative examples} 
    \item Discuss caption-generation methodology; related work on BLIP-2
    \item Discuss how yeah, this means we are still coupled to something that used non-public-domain data.
    \item Summarize why the indirection here is still a benefit (and defer to the Appendix for longer analysis as to why this is something that is reasonable to do, even if not perfect) 
    \item Discuss caption quality? (Only if it's relevant; still not entirely clear to me why this matters so much for the rest of the story, other than intuitively it seems like a good thing) \aaron{BLIP2 have a frozen LLM can explain ow we are able to get better performance on CoCo captions than the ground truth (even using the same data)} 
\end{itemize}




\textbf{5. Testing out the benchmark section}:
\begin{itemize}[topsep=0pt, leftmargin=.5cm]
    \item All experimental details 
    \item Here is where it would be cool to demonstrate trade-offs / considerations via experiments (the stuff that is in Section 9 right now, but really rigorously; let's map this out together?)
    \item Detailed artifact release
\end{itemize}

\textbf{6. Related work and discussion}:
\begin{itemize}[topsep=0pt, leftmargin=.5cm]
    \item Talk about other captioning work
    \item Talk about other open models / licensed models / stuff like that 
    \item Brag about artifact release
\end{itemize}

\textbf{7. Conclusion and future work}:
\begin{itemize}[topsep=0pt, leftmargin=.5cm]
    \item Really cool lessons here
    \item Release really cool artifacts
    \item huge potential for future research, affordances for researchers not at huge labs; this is a new and useful benchmark people should use
    \item This is the baseline for public-domain-trained Stable Diffusion. Can only go up from here, and this should be seen as really exciting / encouraging 
\end{itemize}

==> iclr2023/tables/combined-speedup-table.tex <==
\begin{table}
\centering
\caption{Performance and Approx Cost of Training UNet Cloud}
\label{tab:unet-performance-cost}
\resizebox{\textwidth}{!}{%
\small % or \footnotesize or \tiny, choose the desired font size
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Number of A100s} & \textbf{256x256 (img/s)} & \textbf{512x512 (img/s)} & \textbf{512x512 with EMA (img/s)} & \textbf{Days to Train} & \textbf{Cost(\$)} \\
\hline
%8 & 128.2 & N/A & 258.83 & 258.83 &  \$99,000.00 \\

8  & 1100 & 290  & 290  & 101.04 & \$38,800.00 \\
\hline
%16 & 254.0& N/A  & 130.63 & 130.64&  \$100,000.00 \\

16 & 2180 & 585  & 580  & 50.29  & \$38,630.00 \\
\hline
%32 & 485.7 &N/A & 68.33 & 68.32&  \$105,000.00 \\

32 & 4080 & 1195 & 1160 & 25.01  & \$38,420.00 \\
\hline
%64 & 912.2 &N/A & 36.38 & 36.377 & \$110,000.00 \\

64 & 8530 & 2340 & 2220 & 12.63  & \$38,800.00 \\
\hline
%128 & 1618.4 & N/A & 20.5 & 20.50 & \$125,000.00 \\

128& 11600& 4590 & 3927 & 6.79  & \$41,710.00 \\
\hline
\end{tabular}%
}
\end{table}






% \begin{table}[t]
% \centering
% \caption{Performance and Cost Metrics for U-Net Training on MosaicML Cloud}
% \label{tab:unet-performance-cost}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \textbf{Number of A100s} & \textbf{U-Net @ 256x256 (images / second)} & \textbf{U-Net @ 512x512 (images / second)} & \textbf{U-Net @ 512x512 with EMA (images / second)} & \textbf{Days to Train on MosaicML Cloud} \%& \textbf{Approx. Cost on Cloud} \\
% \hline
% 8  & 1100 & 290  & 290  & 101.04 & \$38,800.00 \\
% \hline
% 16 & 2180 & 585  & 580  & 50.29  & \$38,630.00 \\
% \hline
% 32 & 4080 & 1195 & 1160 & 25.01  & \$38,420.00 \\
% \hline
% 64 & 8530 & 2340 & 2220 & 12.63  & \$38,800.00 \\
% \hline
% 128& 11600& 4590 & 3927 & 6.79   & \$41,710.00 \\
% \hline
% \end{tabular}
% \end{table}


==> iclr2023/tables/dataset-size-table.tex <==
\begin{tabular}{c|c}
    Model & Dataset Size \\
    SD2 & 2,000,000,000 \\
    SDXL & 5,000,000,000 \\
    Ours (LAION) & 1,100,000,000\\
    Ours (YFCC-NC) & ~80 million \\
    Ours (YFCC-COMM) & ~30 million \\
\end{tabular}

==> iclr2023/tables/exact_license_count.tex <==
Attribution-NonCommercial License
12468229
Attribution-NonCommercial-ShareAlike License
28314685
Attribution-NonCommercial-NoDerivs License
25790117
Attribution-NoDerivs License
4827970
Attribution-ShareAlike License
9270079
Attribution License
16962338

==> iclr2023/tables/og-speedup.tex <==

% Number of A100s	Throughput (images / second)	Days to Train on MosaicML Cloud	A100-hours	Approx. Cost on MosaicML Cloud
% 8	128.2	258.83	49,696	$99,000
% 16	254.0	130.63	50,166	$100,000
% 32	485.7	68.33	52,470	$105,000
% 64	912.2	36.38	55,875	$110,000
% 128	1618.4	20.5	62,987	$125,000
% 256*	2,589.4	12.83	78,735	$160,000

\begin{table}[h]
    \centering
    \caption{Performance Metrics on MosaicML Cloud}
    \label{tab:performance_metrics-oh}
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        Number of A100s & Throughput (images / second) & Days to Train on MosaicML Cloud & A100-hours & Approx. Cost on MosaicML Cloud \\
        \hline
        8 & 128.2 & 258.83 & 49,696 & $99,000 \\
        16 & 254.0 & 130.63 & 50,166 & $100,000 \\
        32 & 485.7 & 68.33 & 52,470 & $105,000 \\
        64 & 912.2 & 36.38 & 55,875 & $110,000 \\
        128 & 1618.4 & 20.5 & 62,987 & $125,000 \\
        256* & 2,589.4 & 12.83 & 78,735 & $160,000 \\
        \hline
    \end{tabular}
\end{table}
